The Unreasonable Effectiveness of Deep Features as a Perceptual Metric

While it is nearly effortless for humans to quickly assess the perceptual similarity between two images, the underlying processes are thought to be quite complex. Despite this, the most widely used perceptual metrics today, such as PSNR and SSIM, are simple, shallow functions, and fail to account for many nuances of human perception. Recently, the deep learning community has found that features of the VGG network trained on ImageNet classification has been remarkably useful as a training loss for image synthesis. But how perceptual are these so-called "perceptual losses"? What elements are critical for their success? To answer these questions, we introduce a new dataset of human perceptual similarity judgments. We systematically evaluate deep features across different architectures and tasks and compare them with classic metrics. We find that deep features outperform all previous metrics by large margins on our dataset. More surprisingly, this result is not restricted to ImageNet-trained VGG features, but holds across different deep architectures and levels of supervision (supervised, self-supervised, or even unsupervised). Our results suggest that perceptual similarity is an emergent property shared across deep visual representations.

==> tables/tid2013.tex <==
\begin{table}[t]
\begin{center}
\scalebox{0.85} {
\begin{tabular}{ r c c c } \\
& \textbf{avg} & \textbf{scale} & \textbf{scale \& layer} \\
& & \textbf{oracle} & \textbf{oracle} \\ \hline
SqueezeNet~\cite{iandola2016squeezenet} & .762 & .796 & .813 \\
AlexNet~\cite{krizhevsky2014one} & .811 & \textbf{.841} & \textbf{.851} \\
VGG16~\cite{simonyan2014very} & .707 & .749 & .800 \\
Resnet50~\cite{he2015deep} & .717 & .743 & .765 \\
\hline
FSIMc~\cite{zhang2011fsim} & \textbf{.851} &  &  \\
FSIM~\cite{zhang2011fsim} & .801 &  &  \\
MSSIM~\cite{wang2003multiscale} & .787 & & \\
SSIM~\cite{wang2004image} & .637 &  &  \\
PSNR & .640 &  &  \\
\end{tabular}
}
\label{tab:tid}
\caption{\textbf{TID2013 Results with Pre-Trained Networks}. We show performance of pre-trained classification networks on the TID2013~\cite{ponomarenko2015image} dataset using Spearman correlation with the MOS score provided by the dataset. Each network is run across multiple scales. In the first column, we compute the average cosine distance across all scales and layers. We then assume that the network has a scale oracle, as well as a scale \& best layer oracle in the 2nd and 3rd columns. Note that the deep networks are already highly competitive with designed models.}
\end{center}
\end{table}
